Peek Across: Improving Multi-Document Modeling via Cross-Document Question-Answering

The integration of multi-document pre-training objectives into language models has resulted in remarkable improvements in multi-document downstream tasks. In this work, we propose extending this idea by pre-training a generic multi-document model from a novel cross-document question answering pre-training objective. To that end, given a set (or cluster) of topically-related documents, we systematically generate semantically-oriented questions from a salient sentence in one document and challenge the model, during pre-training, to answer these questions while "peeking" into other topically-related documents. In a similar manner, the model is also challenged to recover the sentence from which the question was generated, again while leveraging cross-document information. This novel multi-document QA formulation directs the model to better recover cross-text informational relations, and introduces a natural augmentation that artificially increases the pre-training data. Further, unlike prior multi-document models that focus on either classification or summarization tasks, our pre-training objective formulation enables the model to perform tasks that involve both short text generation (e.g., QA) and long text generation (e.g., summarization). Following this scheme, we pre-train our model -- termed QAmden -- and evaluate its performance across several multi-document tasks, including multi-document QA, summarization, and query-focused summarization, yielding improvements of up to 7%, and significantly outperforms zero-shot GPT-3.5 and GPT-4.

==> stats/ablation_study.tex <==
\begin{table}[!tb]
    \newcommand{\colindent}{\;}
    \centering
    \resizebox{0.49\textwidth}{!}{
    \begin{tabular}{@{}lrr@{}}
    \toprule
    \phantom{fwidsvhckzxjvchndfzxvvgdaczfc} & Joint & $\Delta$\\
    \midrule
    \textsc{CDLM}-large + $\mathcal{L}_{QE}$ and $sim(\cdot)$ is Eq. \ref{eq:cos_k} & 74.6 & \\
    \colindent $-$ using a single $\tau$ parameter for all the question types & 74.2 & -0.4 \\
    \midrule
    \colindent $-$ $sim(\cdot)$ is the dot product & 73.1 & -1.5\\
    \colindent $-$ $sim(\cdot)$ is the cosine similarity & 74.0 & -0.6\\
    \colindent $-$ $sim_k(\cdot)$ is the bilinear distance (Eq.~\ref{eq:first_s}) & 73.7 & -0.9 \\
    \colindent $-$ $sim(\cdot)$ is Eq.~\ref{eq:cos_k} with a single projection ($W_k=W$) & 74.0 & -0.6 \\
        \midrule
    \colindent $-$ w/o incorrect question type projected negatives & 74.2 & -0.4 \\
    \bottomrule
    \end{tabular}}
    \caption{Similarity function ablation results (Joint $F_1$) of CDLM-large and our loss term on the HotpotQA-distractor dev set.}
    \label{tab:ablations}
\end{table}
